MOHO: Learning Single-view Hand-held Object Reconstruction with Multi-view Occlusion-Aware Supervision

Previous works concerning single-view hand-held object reconstruction typically rely on supervision from 3D ground-truth models, which are hard to collect in real world. In contrast, readily accessible hand-object videos offer a promising training data source, but they only give heavily occluded object observations. In this paper, we present a novel synthetic-to-real framework to exploit Multi-view Occlusion-aware supervision from hand-object videos for Hand-held Object reconstruction (MOHO) from a single image, tackling two predominant challenges in such setting: hand-induced occlusion and object's self-occlusion. First, in the synthetic pre-training stage, we render a large-scaled synthetic dataset SOMVideo with hand-object images and multi-view occlusion-free supervisions, adopted to address hand-induced occlusion in both 2D and 3D spaces. Second, in the real-world finetuning stage, MOHO leverages the amodal-mask-weighted geometric supervision to mitigate the unfaithful guidance caused by the hand-occluded supervising views in real world. Moreover, domain-consistent occlusion-aware features are amalgamated in MOHO to resist object's self-occlusion for inferring the complete object shape. Extensive experiments on HO3D and DexYCB datasets demonstrate 2D-supervised MOHO gains superior results against 3D-supervised methods by a large margin.

==> sections/0abstract.tex <==

%%%%%%%%% ABSTRACT
\begin{abstract}

% Reconstructing hand-held object from a single image is an essential while challenging problem, especially when ground truth 3D object model is unavailable.
% However, utilizing real-world hand-object multi-view images to supervise single-view hand-held object reconstruction network typically faces two core problems: hand-caused occlusion and object self-occlusion.
% In this paper, we present MOHO to simultaneously address such two core problems.
% First, to address the hand-caused occlusion, we develop an occlusion-aware pre-training technique, assisting the network to gain the capability to remove hand occlusion.
% Moreover, we introduce a structural prior extracted by a DINO model pre-trained on large-scale datasets to provide strong part-level semantic information of the object.
% Second, although hand occludes the object, it also provides strong priors to the object shape, which benefits the solution of object self-occlusion.
% We exploit a 3D geometric hand embedding providing cues to complete the invisible object structures using estimated hand joints.
% Extensive experiments on HO3D and DexYCB datasets demonstrate that 2D-supervised MOHO gains superior results against 3D-supervised methods by a large margin.
% Codes will be released soon.


% In this paper, we present MOHO, a novel framework for reconstructing hand-held object from a single image, without leveraging hand-to-collect real-world 3D models for supervision.
% Our approach primarily tackles two predominant challenges insufficiently addressed by earlier techniques: hand-induced occlusion and object's self-occlusion.
% First, we utilize extensive synthetic hand-object videos to pretrain the MOHO model.
% Multi-view occlusion-aware supervision is incorporated to endow the network with the capability to capture hand-object interactions.
% Leveraging the geometric details of the hand and visible object segments, MOHO can discern the shape of areas concealed by the hand.
% Second, as we progress through both pretraining and subsequent fine-tuning phases using real-world data, features derived from camera positions, hand configurations, and pretrained DINO models are amalgamated to maximize the use of all accessible cues
% Extensive experiments on HO3D and DexYCB datasets demonstrate that 2D-supervised MOHO gains superior results against 3D-supervised methods by a large margin.
% Codes will be released soon.

% \iffalse.
% exploit and analyze, aggregate two information
% 首先，我们建立hand-to-object correlation 来恢复被手遮挡住的物体，同时利用手的位姿和几何先验信息， 方法是使用大规模的合成数据集预训练，恢复手的mask, mask 又在实际场景中的手误重建被进一步最为weighting去引导物体的重建。
% 然后，我们建立object-to-object semantic cues. 在大规模的与训练中添加对物体的监督，在实际训练中在结合D I N Ofeature 添加物体的寓意信息。
% \fi

% \iffalse
% In this paper, we present MOHO, a novel framework for reconstructing hand-held object from a single image, without supervision from hard-to-collect real-world 3D models.
% Our approach primarily tackles two predominant challenges when adopting multi-view supervision from real-world hand-object videos: hand-induced occlusion and object's self-occlusion.
% First, hand-to-object correlations are constructed for releasing hand-induced occlusion.
% We leverage the multi-view occlusion-aware supervision on synthetic hand-object videos to pre-train MOHO for the capability to discern and complete the regions of the shape concealed by the hand.
% Auxiliary 2D probabilistic hand occlusion maps are generated for providing hand-to-object correlations when fine-tuning with incomplete real-world observations.
% Second, partial-to-full cues are considered to solve object's self-occlusion. 
% 3D hand articulations implying self-occluded information as well as pre-trained DINO features containing partial-to-full correspondences are amalgamated.
% Extensive experiments on HO3D and DexYCB datasets demonstrate that 2D-supervised MOHO gains superior results against 3D-supervised methods by a large margin.
% Codes will be released soon.
% \fi

Previous works concerning single-view hand-held object reconstruction typically rely on supervision from 3D ground-truth models, which are hard to collect in real world.
In contrast, readily accessible hand-object offer a promising training data source, but they only give partial object observations with complex occlusion.
In this paper, we propose to exploit \textbf{M}ulti-view \textbf{O}cclusion-aware supervision from hand-object videos for \textbf{H}and-held \textbf{O}bject reconstruction (MOHO) from a single image, tackling two predominant challenges including object's self-occlusion and hand-induced occlusion.
MOHO inputs semantic features indicating visible object parts and geometric embeddings provided by hand articulations as partial-to-full cues to resist object's self-occlusion, so as to recover the full shape of the object.
Meanwhile, a novel 2D-3D hand-occlusion-aware training scheme following the synthetic-to-real paradigm is proposed to address hand-induced occlusion.
In the synthetic pre-training stage, 2D-3D hand-object correlations are constructed by supervising MOHO with rendered images to complete the hand-concealed regions of the object in both 2D and 3D spaces.
Subsequently, MOHO is finetuned in real world by the amodal-mask-weighted supervision adopting hand-object correlations obtained during the pre-training.
Extensive experiments on HO3D and DexYCB datasets demonstrate that 2D-supervised MOHO attains superior results against 3D-supervised methods by a large margin.
Codes and key assets will be released soon.

% In this paper, we present MOHO, a novel synthetic-to-real domain adaptation framework for reconstructing hand-held object from a single image, without using supervision from hard-to-collect real-world 3D models.
% MOHO mainly tackles two predominant challenges that are insufficiently addressed by previous methods: hand-induced occlusion and object's self-occlusion.
% First, in the synthetic training stage, we render large-scale paired images with one capturing target hand-held object and the other describing the complete object.
% MOHO takes the paired images, hand pose and shape embeddings, DINO features as input to recover complete 2D mask and 3D shape of the object respectively, under the supervision of our occlusion-aware consistency terms.
% In this manner, prior knowledge from the hand and visible object parts is well exploited.
% Second, in the real-world adaptation stage, we freeze the 2D mask recovery branch due to its cross-domain consistency.
% We finetune MOHO harnessing mask-weighted volume rendering supervision to narrow the domain gap in 3D shape.
% Extensive experiments on HO3D and DexYCB datasets demonstrate that 2D-supervised MOHO gains superior results against 3D-supervised methods by a large margin.
% Codes will be released soon.

% In this paper, we present a novel synthetic-to-real domain adaptation framework to exploit \textbf{M}ulti-view \textbf{O}cclusion-aware supervision from hand-object videos for \textbf{H}and-held \textbf{O}bject reconstruction (MOHO) from a single image, without using supervision from hard-to-collect real-world 3D models.
% MOHO mainly tackles two predominant challenges in such setting: hand-induced occlusion and object's self-occlusion.
% First, in the synthetic pre-training stage, we render a large-scale synthetic dataset OMVideo with multi-view hand-object images and occlusion-free supervisions.
% MOHO inputs the hand-object reference image, and extracts domain-consistent parital-to-full cues to resist object's self-occlusion, finally recovers 2D amodal mask and 3D complete shape of the object respectively.
% The rendered occlusion-free supervisions are used in this stage to address hand-induced occlusion in both 2D and 3D spaces.
% Second, in the adaptation stage, MOHO is finetuned by the additional amodal-mask-weighted geometric supervision generated by the frozen 2D amodal mask recovery head, to mitigate the negative effects caused by hand-occluded supervision views in real world.
% Extensive experiments on HO3D and DexYCB datasets demonstrate that 2D-supervised MOHO gains superior results against 3D-supervised methods by a large margin.
% Codes will be released soon.

\end{abstract}

==> sections/1intro.tex <==
\section{Introduction}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{figures/Teaser.pdf}
    \caption{
    During the real-world training, MOHO is only supervised by the occluded hand-object videos . 
    In the testing stage, MOHO generates complete object novel views as well as photorealistic reconstructed mesh, resisting hand-induced occlusion and object's self-occlusion.}
    \label{fig:teaser}
\vspace{-0.7cm}
\end{figure}

Understanding hand-object interaction is becoming increasingly important in many practical scenarios including robotics \cite{zheng2023cams,li2020hoi}, augmented and virtual reality \cite{leng2021stable}, as well as embodied artificial intelligence systems \cite{xu2023unidexgrasp,li2023behavior}.
Although there exist previous works \cite{chao2021dexycb,hampali2020honnotate,yang2022oakink} aiming at reconstructing fine hand-held object meshes from multi-view image sequences, single-view methods \cite{ye2022s,chen2022alignsdf,chen2023gsdf, hasson2019learning, karunratanakul2020grasping,zhang2023ddf} are drawing more attention recently since they can be applied more conveniently in real-world environment.

Given the ill-posed nature of single-view reconstruction, current top-preforming methods \cite{ye2022s,chen2022alignsdf,chen2023gsdf} typically use Signed Distance Field (SDF) as geometric representation and employ 3D ground-truth meshes as supervision for training.
However, the applicability of such an approach in real-world scenarios is highly challenging, as obtaining clean and precise object meshes remains a formidable task.
In contrast, readily accessible raw videos capturing hands interacting with objects offer a promising training data source. 
Nevertheless, leveraging these videos as multi-view supervision for single-view hand-held object reconstruction introduces two significant challenges: hand-induced occlusion and object's self-occlusion. 
As the hands manipulate the objects, hand-induced occlusion is inevitable in our easily obtained training data, leading to omnipresently incomplete object masks for multi-view supervision.
This incompleteness poses a significant barrier for the network to effectively learn the reconstruction of the complete object shape.
Moreover, object's self-occlusion arises due to the single-view setting. 
With only one reference view provided, the visible area of the object remains incomplete, further complicating the task of recovering the object's full shape for the network.

To address the aforementioned problems, we propose MOHO with \textbf{M}ulti-view \textbf{O}cclusion-aware supervision for single-view \textbf{H}and-held \textbf{O}bject reconstruction (\cref{fig:teaser}).
MOHO incorporates both semantic features and geometric hand articulation embeddings to resist the object's self-occlusion caused by the only reference view.
The semantic features present significant partial-to-full cues for MOHO by indicating which portions are visible in the reference view and identifying the areas requiring reconstruction to generate the complete shape.
The geometric embeddings further guide MOHO to hallucinate the shape of the occluded surfaces hinted by the hand's holding pose.
Equipped with such information, the geometric volume rendering technique is adopted in MOHO to generate the complete object novel views as well as the photorealistic reconstructed mesh of the hand-held object.
To mitigate the challenges posed by hand-induced occlusion, we propose a novel 2D-3D hand-occlusion-aware training scheme following the synthetic-to-real paradigm.
Specifically, MOHO is first pre-trained with rendered large-scale paired images, with one capturing the target hand-held object as input and the other describing the complete object in a novel view as supervision.
Thus, MOHO is empowered to grasp hand-object correlation in 3D space so as to remove hand-induced occlusion.
Simultaneously, an auxiliary 2D hand cover segmentation head is integrated into the pre-training process, which predicts the hand-occluded parts of the object in the reference view.
The predictions from this 2D head are subsequently employed during the real-world finetuning stage to establish the amodal-mask-weighted supervision, designed to combat the challenges presented by real-world hand-induced occlusion.

To summarize, our main contributions are threefold:
\begin{itemize}
    \item We propose MOHO to pursue photorealistic hand-held object reconstruction from a single-view image without relying on 3D ground-truth supervision.
    Adequate semantic features and geometric embeddings are utilized as partial-to-full cues for solving the object's self-occlusion problem.
    \item 
    We present a novel 2D-3D hand-occlusion-aware training scheme to release the hand-induced occlusion.
    The 2D-3D hand-object correlations are constructed in the pre-training stage and the amodal-mask-weighted supervision is used in the real-world finetuning stage.
    \item 
    Extensive experiments on real-world datasets HO3D~\cite{hampali2020honnotate} and DexYCB~\cite{chao2021dexycb} demonstrate that 2D-supervised MOHO gains superior results against 3D-supervised methods by a large margin.
\end{itemize}

==> sections/3method.tex <==
\section{Method}
\subsection{Overview}
As shown in \cref{fig:pipeline}, given a single input reference image $\mathcal{I}$ depicting hand-object interaction, its corresponding camera pose $\mathcal{P}_I$ (I-1), offline-estimated hand-object segmentation $\mathcal{S}_h$, $\mathcal{S}_o$, and hand pose prediction $\theta_A$ (I-2), MOHO synthesizes novel views as well as the textured mesh of the complete hand-held object.
Specifically, MOHO first utilizes a CNN-based encoder $\phi$ to extract color features $\mathcal{F}_c$ (N-1) of the input segmented image with the occluded object $\mathcal{I}\odot\mathcal{S}_o$.
Meanwhile, the semantic hints $\mathcal{F}_s$ (N-2), extracted by a pre-trained DINO~\cite{amir2022effectiveness} model $\mathcal{D}$, offer the network partial-to-full correspondences for perceiving the amodal object shape.
Furthermore, 3D geometric hand articulation embeddings $\mathcal{F}_h$ (N-3) are amalgamated to provide geometry information for MOHO to recover the unseen surfaces of the single reference view.
Finally, such semantic and geometric features $\mathcal{F}_c$, $\mathcal{F}_s$ and $\mathcal{F}_h$ are concatenated as the condition for the geometric volume rendering heads~\cite{wang2021neus} $\psi_S$, $\psi_C$ (N-4) to predict SDF value and color density respectively, enabling reconstruction of the agnostic occluded hand-held object without any instance priors.
% For the volume rendering head, referring to \cite{wang2021neus}, two volume rendering heads $\psi_S$, $\psi_C$ predicting SDF value and color density respectively are adopted.
% Given semantic and geometric features with partial-to-full cues, the volume rendering heads generate complete novel views as well as the photorealistic mesh of the occluded hand-held object in the single reference view.

Since real-world hand-object videos only contain incomplete object observations under heavy hand-induced occlusion, extra supervision needs to be introduced to guide MOHO to recover the hand-concealed regions of the object.
Thus, we propose an elaborated 2D-3D \textbf{H}and-\textbf{O}cclusion-\textbf{A}ware (HOA) training scheme for handling hand-induced occlusion, which is developed on the basis of synthetic-to-real transferring.
The HOA training procedure includes 2D-3D \textbf{H}and-\textbf{O}bject \textbf{C}orrelation (HOC) pre-training (T-1) and real-world finetuning (T-2) with amodal-mask-weighted supervision.
% First, MOHO is pre-trained on synthetic hand-object video clips for constructing 3D hand-object correlations, with hand-occluded incomplete object images as inputs and full-object images as novel-view supervision.
% Meanwhile, a 2D auxiliary segmentation head is also pre-trained for predicting 2D probabilistic hand occlusion maps, indicating the projection of the object parts occluded by hands inferred by incomplete observations.
% Afterwards, the 2D auxiliary head is transferred to real world data, whose probabilistic predictions are utilized as the mask-weighted supervision for the real-world finetuning of MOHO.
Such HOA training endows MOHO to transfer the pre-learned hand-removal knowledge for completing the hand-occluded object shape in real world.


\subsection{Partial-to-full Cues for Geometric Volume Rendering}
\label{cues}

Generating novel views and full mesh for the object given by the only reference view is typically an ill-posed problem due to severe object's self-occlusion.
Hence, besides the color features $\mathcal{F}_c$ (Fig. \ref{fig:pipeline} (N-1)), we need to feed sufficient information to the network for completing the unobserved area in the reference image.
We consider the partial-to-full cues from two aspects: semantic hints and geometric embeddings.
The DINO features $\mathcal{F}_s$ (Fig. \ref{fig:pipeline} (N-2)) are used as the semantic hints since they consist of the global consistent information of the object learned from large-scale pre-training.
Therefore, $\mathcal{F}_s$ helps the network discern which parts are observed and guides the volume rendering heads to generate the unseen regions.
On the other hand, the geometric embeddings $\mathcal{F}_h$ (Fig. \ref{fig:pipeline} (N-3)) obtained from the predicted hand articulations are considered.
Given the knowledge that the local joints' distribution of the holding hand implies the held object's shape, $\mathcal{F}_h$ assists MOHO in perceiving the unobserved object surfaces at 3D level.
Semantic and geometric features $\mathcal{F}_s$ and $\mathcal{F}_h$ provide partial-to-full cues for the subsequent geometric volume rendering heads to overcome the object's self-occlusion caused by the single-view setting.

\nbf{Color Features}
Previous works~\cite{yu2021pixelnerf,jang2021codenerf,chen2023single,lin2023vision,xu2022sinnerf} have demonstrated that suitable conditional color features on volume rendering heads benefit the scenarios given only one or sparse input views.
Since MOHO needs to handle the single-view reconstruction task, we follow \cite{yu2021pixelnerf} to use a ResNet34~\cite{he2016deep} as the image encoder $\phi$ to extract the hand-held object color feature map $\mathcal{F}^I_c = \phi(\mathcal{I}\odot\mathcal{S}_o)$ of the reference view $\mathcal{I}$.
Since MOHO adopts the volume rendering technique, the feature map $\mathcal{F}^I_c$ needs to be converted to the features corresponding to the 3D sampled points.
Given the camera poses $\mathcal{P}_I$ and camera parameters $\mathcal{K}$, 3D points $\{P_i\}_{i=1}^n$ along the sampled rays are first projected onto the image plane and get the corresponding pixel positions.
The patched color features of each sampled point $\mathcal{F}^i_c$ are fetched on $\mathcal{F}^I_c$ via bilinear interpolation.

\nbf{Semantic Hints}
% Considering object's self-occlusion, MOHO needs to know what parts of the object are seen so that it can better perceive the full object shape.
The semantic hints $\mathcal{F}_s$ are exploited to provide MOHO with high-level information containing structural priors for amodal object perception.
Concretely, we harness semantic descriptors from the pre-trained DINO~\cite{amir2022effectiveness}, which provides local descriptors with consistent structural information to indicate the position of the observed object parts within the whole shape.
With such clues, MOHO learns to complement the full object better when only the occluded observation is given. 
Specifically, the pre-trained DINO model $\mathcal{D}$ extracts the patch-wise feature maps $\mathcal{F}^I_s = \mathcal{D}(\mathcal{I})\odot\mathcal{S}_o$.
We use the top three principal components of $\mathcal{F}^I_s$ by principal component analysis (PCA) considering the trade-off between efficiency and performance, and unsample them into the same resolution as $\mathcal{F}^I_c$.
The $\mathcal{F}^i_s$ of the sampled 3D point $P_i$ is obtained by the same projection and interpolation operations as the generation of $\mathcal{F}^i_c$.

\nbf{3D Hand Articulation Embeddings}
3D hand articulation embeddings are adopted for providing 3D geometric guidance for MOHO to overcome object's self-occlusion caused by the single-view degeneration.
As \cite{xu2022sinnerf} demonstrates, reconstructing the whole scene from a single reference view may make the volume rendering technique prone to generate unsatisfactory results, whose surface toward the reference view is recovered decently, but the reconstruction of unseen parts is typically degraded.
Considering that the holding hand shape implies the unobserved hand-held object shape, we add 3D hand articulation embeddings $\mathcal{F}^i_h$ for each sampled point $P_i$.
Notably, we treat the hand articulation locally rather than globally as the previous methods \cite{ye2022s,chen2023gsdf} do.
This is due to our motivation that using 3D hand articulations is to guide the unobserved parts' completion.
For the specific unseen part, the most credible heuristics implied by the holding hand shape come from the nearest hand joints' positions.
Taking all the joints' coordinates is unnecessary and leads to more complexity, as demonstrated by the ablations in Sec. \ref{ablation}. 
Therefore, the adopted 3D hand articulation embeddings explicitly represent the geodesic distances from the sampled point $P_i$ to the nearest hand joints.
Specifically, we first use an off-line hand pose estimator to get hand articulation parameter $\theta_A$ from the reference image. 
Then, we run forward kinematics of MANO model~\cite{romero2022embodied} to derive the transformation $T(\theta_A)$ as well as the hand joint coordinates.
After selected by the K-nearest-neighbors, the sampled point $P_i$ is mapped to the nearest $K$ hand joint coordinates by their transformation matrices. 
Finally, such $K$ positions of the sampled point in the nearest $K$ hand joint coordinates are concatenated as $\mathcal{F}^i_h$ to provide the distance information.
We select $K=6$ during the implementation.

\nbf{Conditional Geometric Volume Rendering}
After incorporating all the partial-to-full cues, we construct the conditional geometric volume rendering technique to render novel views as well as generate textured meshes (Fig. \ref{fig:pipeline} (N-4)).
Specifically, given 3D sampled points $\{P_i\}$, ray directions $\{D_i\}$ and corresponding point features $\{\mathcal{F}_i\} = \text{Concat}(\mathcal{F}^i_c, \mathcal{F}^i_c, \mathcal{F}^i_h)$ extracted from the single reference view $\mathcal{I}$, a geometric field $\psi_S$ predicting the SDF value $s_i = \psi_S(P_i | \mathcal{F}_i)$ as well as a color field $\psi_C$ predicting the RGB density $c_i = \psi_C(P_i, D_i | \mathcal{F}^i_c)$ are constructed. 
As for volume rendering, 3D points $\{P_i\}$ are sampled along camera rays by $\{P\}$ = $\{P(z) | P(z) = O + zD, z \in [z_n, z_f]\}$, where $O$ denotes the origin of the camera, $D$ refers to the viewing direction of each pixel, $z_n$, $z_f$ are the near and far bounds of the ray.
$O$ and $D$ are calculated by the input camera pose $\mathcal{P}_I$ and camera intrinsic $\mathcal{K}$.
Then, the color of the pixel is rendered by
\begin{equation}
\hat{c} = \int_{z_n}^{z_f} \omega(z) \psi_C(P(z), D | \mathcal{F}^C) dz,
\end{equation}
where $\omega(z) = T(z) \rho(z)$ is an unbiased and occlusion-aware function proposed by \cite{wang2021neus}, converting SDF value $\psi_S(P | \mathcal{F})$ to $T(z), \rho(z)$ by
\begin{equation}
T(z) = \exp\left(-\int_{z_n}^{z_f}\rho(z)dz\right),
\end{equation}
\begin{equation}
\rho(z) = \max\left(\frac{-\frac{d \sigma^h}{dz}\left(\psi_S(P(z) | \mathcal{F})\right)}{\sigma^h\left(\psi_S(P(z) | \mathcal{F})\right)},0\right).
\end{equation}
$\sigma^h$ here denotes the Sigmoid function with a trainable parameter $h$.
During implementation, the formulations above are numerically discretized as referred to \cite{wang2021neus}.

\subsection{2D-3D Hand-Occlusion-Aware Training}
\label{training}
The previous 3D supervised work \cite{ye2022s} utilizes the synthetic dataset containing large amounts of objects to enhance the performance on real-world data.
We take a further step by adopting the synthetic dataset to conduct 2D-3D Hand-Occlusion-Aware (HOA) training, releasing the problem that real-world training data is partially observed and heavily occluded by hands.
The 2D-3D HOA training encompasses two stages, \ie, 2D-3D Hand-Object Correlation (HOC) pre-training, and real-world finetuning with amodal-mask-weighted supervision.

In the 2D-3D HOC pre-training stage, we foster MOHO for the capability to be aware of the hand-occluded regions of the object in both 3D and 2D spaces.
For 3D hand-object correlation construction, MOHO inputs the hand-occluded reference view $\mathcal{I}\odot\mathcal{S}_o$, extracts the proposed partial-to-full cues for the volume rendering head, and is supervised by the synthetic complete object in a novel view.
Further, an auxiliary 2D hand concealment segmentation head incorporating the same partial-to-full cues is utilized to predict the probabilistic hand occlusion map from $\mathcal{I}\odot\mathcal{S}_o$.

After pre-training, MOHO is finetuned with real-world hand-object videos.
However, real-world hand-object multi-view images oftentimes only contain truncated regions and incomplete views, resulting in detrimental effects when directly used for training.
Naively utilizing the defective masks of the hand-occluded objects misleads the network to reconstruct patchy geometric surfaces.
Thus, the predictions from the pre-trained 2D hand concealment segmentation head are leveraged on real-world data.
Together with the observed incomplete object masks, we construct a soft constraint and introduce the amodal-mask-weighted supervision for reconstructing full hand-held object shapes. 

\nbf{2D-3D Hand-Object Correlation Pre-Training}
MOHO is first enabled to remove hand-induced occlusion in 3D space by the rendered occlusion-free supervision.
Concretely, the input reference view fed to MOHO is an image with hand-object interaction, while the supervision view is a rendered full-object picture from a novel pose.
Referring to the construction pipeline of ObMan~\cite{hasson2019learning} dataset, we render an amount of hand-object video clips by setting up the hand-object interaction scenes and moving them.
First, we select the same objects as ObMan from the ShapeNet dataset~\cite{chang2015shapenet}.
Objects' textures are randomly sampled from the texture maps provided by ShapeNet.
Then, the grasping generation procedure adopting GraspIt~\cite{miller2004graspit} is used for the hand-object interaction scene setup.
Finally, we add global rotations and translations on the SMPL+H model~\cite{loper2015smpl,romero2022embodied} to simulate the hand and body motion in real-world hand-object video.
Thus, a synthetic video clip with multi-view information depicting a hand-object interaction scene is generated.
Besides, to enable occlusion-free supervision, we also render corresponding video clips containing only objects without hands and bodies by using the same rotations and translations as above.
During the pre-training, one random view picked from the hand-object video is fed to MOHO, while 8 novel views sampled from the corresponding occlusion-free video are regarded as supervision.
With such supervision, MOHO is capable of constructing hand-object correlation in 3D space, hence removing the hand-induced occlusion.
For more rendering details, please refer to the \supp.

Several losses are designed for supervising MOHO to get geometric consistent surfaces as well as photorealistic novel view synthesis results.
The total loss function is defined as
\begin{equation}
\mathcal{L} = \mathcal{L}_{color} + \lambda_1 \mathcal{L}_{eik} + \lambda_2 \mathcal{L}_{mask} + \lambda_3 \mathcal{L}_{n_{ori}} + \lambda_4 \mathcal{L}_{n_{smo}}.
\label{total_loss}
\end{equation}
The color loss $\mathcal{L}_{color}$ is defined as $\mathcal{L}_{color} = \frac{1}{m} \sum_i |\hat{c}_i - c_i|$, where $m$ is the number of sampling rays.
The Eikonal regularization term $\mathcal{L}_{eik}$ \cite{gropp2020implicit} is added by $\mathcal{L}_{eik} = \frac{1}{nm} \sum_{i,j} (||\nabla \psi_S(P_{i,j})||_2 - 1)^2$, in which $n$ is the number of sampling points along each ray.
At the pre-training stage, the mask loss $\mathcal{L}_{mask}$ is defined as
\begin{equation}
\mathcal{L}_{mask} = BCE(M_i^{co}, \hat{O}_i),
\label{mask_loss}
\end{equation}
where $\hat{O}_i$ is the sum of weight $\omega(z)$ along the ray, and $M_i^{co}$ refers to the rendered complete object mask without hand-induced occlusion.
Two additional losses regularizing the predicted surface normals are used for restricting the orientation of visible normals towards the camera ($\mathcal{L}_{n_{ori}}$) \cite{verbin2022ref} and making the predictions smoother ($\mathcal{L}_{n_{smo}}$) \cite{sharma2021point}, which are detailed in the \supp.
The weighted factors are set to $\lambda_1 = 1.0$, $\lambda_2 = 1.0$, $\lambda_3 = 10^3$, $\lambda_4 = 10^{-2}$ during implementation.
All factors are utilized in both pre-training and real-world finetuning.

Simultaneously, an auxiliary 2D hand concealment segmentation head is utilized in the pre-training to construct 2D hand-object correlation.
The 2D segmentation head, whose architecture refers to \cite{chen2017rethinking}, predicts the 2D projection of the hand-concealed object's part $\hat{M}_I^{ho}$ by the same partial-to-full cues extracted from $\mathcal{I}\odot\mathcal{S}_o$.
The auxiliary supervision is enforced by the binary cross-entropy loss between $\hat{M}_I^{ho}$ and $M_I^{co} \ominus M_I$, where $M_I^{co}$ means the rendered complete mask of the input reference view $\mathcal{I}$, and $M_I$ refers to the input incomplete object mask.
The benefits of incorporating such 2D head are twofold.
\textbf{First}, 2D hand occlusion perception helps construct 2D hand-object correlation.
The auxiliary 2D supervision strengthens the ability of MOHO to handle hand-induced occlusion patterns.
\textbf{Second}, considering more cross-domain consistency of the 2D neural network \cite{cardace2023exploiting}, we exploit the predictions of this 2D segmentation head for the real-world training stage to promote the transferring of the knowledge about hand-object correlations learned in the pre-training stage.
We freeze the 2D segmentation head during the real-world finetuning stage, and infer the probabilistic likelihood maps of hand-concealed object parts (\cref{fig:pipeline} (T-1)).
The likelihood maps are regarded as the relaxed constraints for the proposed amodal-mask-weighted real-world finetuning.
Such information is the effective replenishment of the incomplete masks in real-world supervision caused by hand-induced occlusion.

\nbf{Real-World Finetuning with Amodal-Mask-Weighted Supervision}
After pre-training, MOHO is finetuned on hand-object videos from real-world datasets which typically suffer from partial observations caused by hand-induced occlusion.
Therefore, we introduce the amodal-mask-weighted supervision, taking the probabilistic maps of hand-concealed object's parts predicted by the pre-trained 2D segmentation head into consideration (\cref{fig:pipeline} (T-2)).
The amodal-mask-weighted loss is defined by
\begin{equation}
\mathcal{L}_{mw} = BCE(\hat{M}_i^{ho}\oplus M_i, \hat{O}_i),
\end{equation}
where $\hat{M}_i^{ho}$ is the hand-concealed part prediction by the auxiliary segmentation head and $M_i$ is the incomplete input object segmentation.
The $\mathcal{L}_{mw}$ is the substitution of $\mathcal{L}_{mask}$ defined in \cref{mask_loss}, and it is included in \cref{total_loss} with the same weight factor during the real-world finetuning.
Having gained knowledge about how to handle hand occlusion with such supervision, MOHO is capable of generating novel views of the complete object in real-world scenarios.


